Monotones in General Resource Theories

A central problem in the study of resource theories is to find functions that are nonincreasing under resource conversions - termed monotones - in order to quantify resourcefulness. Various constructions of monotones appear in many different concrete resource theories. How general are these constructions? What are the necessary conditions on a resource theory for a given construction to be applicable? To answer these questions, we introduce a broad scheme for constructing monotones. It involves finding an order-preserving map from the preorder of resources of interest to a distinct preorder for which nontrivial monotones are previously known or can be more easily constructed; these monotones are then pulled back through the map. In one of the two main classes we study, the preorder of resources is mapped to a preorder of sets of resources, where the order relation is set inclusion, such that monotones can be defined via maximizing or minimizing the value of a function within these sets. In the other class, the preorder of resources is mapped to a preorder of tuples of resources, and one pulls back monotones that measure the amount of distinguishability of the different elements of the tuple (hence its information content). Monotones based on contractions arise naturally in the latter class, and, more surprisingly, so do weight and robustness measures. In addition to capturing many standard monotone constructions, our scheme also suggests significant generalizations of these. In order to properly capture the breadth of applicability of our results, we present them within a novel abstract framework for resource theories in which the notion of composition is independent of the types of the resources involved (i.e., whether they are states, channels, combs, etc.).

==> sections/Resource_Types.tex <==
\section{Resource Types}
\label{sec:Resource types}

	In most interesting resource theories, one can identify different types of resources.
	For example, in resource theories of quantum states, we could classify states by the system they are defined on.
	States on different systems would correspond to resources of different types.
	If the different systems involved are discrete, they can be characterized by their Hilbert space dimension, and we get types of resources that are natural numbers.
	This notion of resource types features in quantum resource theories of states and stochastic resource theories of states, arguably the two most prominent classes of resource theories in the literature.
	In other situations, e.g., when we study thermodynamics as a resource theory \cite{Gour2015}, we might distinguish resources pertaining to systems with different Hamiltonians as distinct types of resources.
	If we are interested in asymmetry properties as a resource theory \cite{Marvian2013}, we can label resource types by the relevant group actions.
	
	Another possible distinction between types of resources arises when one is interested in a resource theory that describes states, channels, and possibly other higher order processes in a unified way.
	The types of resources would then also carry information about the inputs and outputs of such processes.
	If one also wanted to impose compatibility of processes with certain causal structure, types like the ones introduced in~\cite{kissinger2017categorical} would become relevant.
	
	Once we introduce types of resources, the set of all resources $R$ is a disjoint union of sets of resources of a particular type.
	Let's denote the set of all types in a resource theory by $\mathrm{ob}(R)$.
	For a type $\alpha \in \mathrm{ob}(R)$, $R[\alpha]$ denotes the set of resources of that type.
	Then, we have
	\begin{equation}
		R = \bigsqcup_{\alpha \in \mathrm{ob}(R)} R[\alpha].
	\end{equation}
	
	In a resource theory with well-defined resource types, we would like the types of resources in the set $r \boxtimes s$ to only depend on the types of $r$ and $s$ rather than the identity of the particular resources $r$ and $s$.
	In order to express this property, we need to specify a list of types that appear in the set of resources $r \boxtimes s$ and therefore we need this set to be indexed.
	With this in mind, we introduce the following notion of a listable resource theory (see also \cite{Gonda2021}).
	\begin{definition}\label{def:listable_ucrt}
		A (universally combinable) resource theory $\RT{R}$ is termed \textbf{listable} if there is a set $\mathcal{I}$ such that for all $r,s \in R$ we have
		\begin{equation}
			\label{eq:listable_star}  
			r \boxtimes s &= \bigcup_{i \in \mathcal{I}} s \boxtimes_i t 
		\end{equation}
		where each $s \boxtimes_i t$ and each $t \apply_i x$ is either a singleton or an empty set.
		Furthermore, we require that for all $i \in \mathcal{I}$ we have
		\begin{equation}\label{eq:listable_associativity}
			(r \boxtimes_i s) \boxtimes_i t &= r \boxtimes_i (s \boxtimes_i t)  
		\end{equation}
		so that each $(R, \boxtimes_i)$ is a semigroup.
	\end{definition}
	\begin{definition}\label{def:listable_ucrt}
		A (universally combinable) resource theory $\RT{R}$ is termed \textbf{listable} if there is a set $\mathcal{I}$ such that for all $r,s \in R$ we have
		\begin{equation}
			\label{eq:listable_star}  
			r \boxtimes s &= \bigcup_{i \in \mathcal{I}} r \star_i s 
		\end{equation}
		where each $s \boxtimes_i t$ and each $t \apply_i x$ is either a singleton or an empty set.
		Furthermore, we require that for all $i \in \mathcal{I}$ we have
		\begin{equation}\label{eq:listable_associativity}
			(r \star_i s) \star_j t &= r \star_i (s \star_j t)  
		\end{equation}
		so that, in particular, each $(R, \star_i)$ is a semigroup.
	\end{definition}
	Note that in general, $\star_i$ is not going to be a commutative operation, which is why we do not denote it by $\boxtimes$ here.
	
	In a resource theory with types it makes sense to allow the index set $\mathcal{I}$ to vary according to the types of the two resources $r,s$.
	We can then express the compatibility of resource combination operation $\boxtimes$ with resource types as follows.
	For any two types $\alpha, \beta \in \mathrm{ob}(R)$, we require that there is %a set $\mathcal{I}_{\alpha,\beta}$ such that for all $r \in R[\alpha]$ and all $s \in R[\beta]$ we have
%	\begin{equation}
%		\label{eq:listable_star_2}  
%		r \boxtimes s &= \bigcup_{i \in \mathcal{I}_{\alpha,\beta}} r \star_i s 
%	\end{equation}
	an indexed family $\mathcal{I}_{\alpha,\beta}$ of types from $\mathrm{ob}(R)$, which represents the unique sequence 
		of types of resources present in the set $r \boxtimes s$ for any $r \in R[\alpha]$ and any $s \in R[\beta]$.
	\togo{However, I still don't know how to make this properly formal.
	We may need, for each triple $r,s,t$ a bijection $(r \boxtimes s) \boxtimes t \to r \boxtimes (s \boxtimes t)$ that acts like an associator.
	There should be a categorical way to do this, also with types, but I just don't see it clearly atm.}
	Formally, $\mathcal{I}_{\alpha,\beta}$ is a function $\omega_{\alpha,\beta} \to \mathrm{ob}(R)$ for a finite cardinal number $\omega_{\alpha,\beta} = \{0,1,\ldots,n-1\}$ with $n$ denoting the 
		number of ways in which resources of type $\alpha$ can be combined with resources of type $\beta$, such that for any $r \in R[\alpha]$ and any $s \in R[\beta]$ we have
	\begin{equation}
		\label{eq:Type compatible operation}
		r \boxtimes s = \Set{ r \boxtimes_{i} s \given  i \in \omega_{\alpha,\beta} },
	\end{equation}
	where $r \boxtimes_{i} s \in R[\mathcal{I}_{\alpha,\beta}(i)]$ is a single resource of type $\mathcal{I}_{\alpha,\beta}(i)$.
	One can thus think of $\boxtimes_{i}$ as a binary operation $R[\alpha] \times R[\beta] \to R[\mathcal{I}_{\alpha,\beta}(i)]$.
	However, note that $\boxtimes_{i}$ is in general not commmutative, \mbox{unlike $\boxtimes$}. 
	
	A resource theory $\RT{R}$ with types $\mathrm{ob}(R)$ is called \textbf{type-compatible} if $\boxtimes$ is compatible with the resource types in the sense described in equation (\ref*{eq:Type compatible operation}).
